Implementation of Two Layers Type Theory in Dedukti and Application to Cubical Type Theory

In this paper, we make a substantial step towards an encoding of Cubical Type Theory (CTT) in the Dedukti logical framework. Type-checking CTT expressions features a decision procedure in a de Morgan algebra that so far could not be expressed by the rewrite rules of Dedukti. As an alternative, 2 Layer Type Theories are variants of Martin-L\"of Type Theory where all or part of the definitional equality can be represented in terms of a so-called external equality. We propose to split the encoding by giving an encoding of 2 Layer Type Theories (2LTT) in Dedukti, and a partial encoding of CTT in 2LTT.

==> eptcsdata.tex <==
\providecommand{\firstpage}{54}
\providecommand{\publicationstatus}{C. Sacerdoti Coen, A. Tiu (Eds.): 15th International Workshop\\ on Logical Frameworks: Theory and Practice (LFMTP 2020)\\
EPTCS 332, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.332.4}{10.4204/EPTCS.332.4}}

